Reining in Mobile Web Performance with Document and Permission Policies

The quality of experience with the mobile web remains poor, partially as a result of complex websites and design choices that worsen performance, particularly for users in suboptimal networks or devices. Prior proposed solutions have seen limited adoption due in part to the demand they place on developers and content providers, and the performing infrastructure needed to support them. We argue that Document and Permissions Policies -- an ongoing effort to enforce good practices on web design -- may offer the basis for a readily-available and easily-adoptable solution. In this paper, we evaluate the potential performance cost of violating well-understood policies and how common such violations are in today's web. Our analysis show, for example, that controlling for unsized-media policy, something applicable to 70% of the top-1million websites, can indeed reduce Cumulative Layout Shift metric.

==> preamble/preamble-acm.tex <==
% Copyright
%\setcopyright{none}
% %\setcopyright{rightsretained}

% % DOI
% %\acmDOI{10.475/123_4}

% % ISBN
% %\acmISBN{123-4567-24-567/08/06}

%Conference
%\acmConference[WWW 2021]{The Web Conference 2021}{April 2021}{Ljubljana, Slovenia}
%\acmYear{2021}
%\copyrightyear{2021}
%\acmArticle{4}
%\acmPrice{15.00}

% DOI
%\acmDOI{10.475/123_4}
% ISBN
%\acmISBN{123-4567-24-567/08/06}
% %Conference
% \acmConference[IMC 2020]{Internet Measurement Conference 2020}{October 2020}{Pittsburgh, PA, USA}
% \acmYear{1997}
% \copyrightyear{2020}
% %\acmArticle{4}
% %\acmPrice{15.00}

% Packages go here
\usepackage{gensymb}
\usepackage{pbox}
\usepackage{subfigure}
\usepackage{epsfig,endnotes}
\usepackage{epstopdf}
\usepackage{times}
\usepackage{color}
\usepackage{colortbl} % to allow background color in the table
\usepackage{graphicx}
\usepackage{xspace}
\usepackage{enumitem}
\usepackage{multirow}
\usepackage{tikz}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
%\usepackage{balance,lastpage}  % to balance last page
\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}


==> sections/dataset.tex <==
\section{Test configuration}
\label{sec:config}

In this section, we introduce how we can achieve our goal, building a readily deployable and extensible performance analysis system for in-the-wild experimentation with different PFP features with a given con-dition, to boost mobile web performance. This will address the virtually infinite combination of countless webpages designs, diverse user devices 1, and network conditions.

4.1	Dataset and metrics

Performance testing with synthetic pages would not reflect such unlimited conditions in the real world. There-fore, we will collect and examine various webpages in the wild in this study. In particular, AMP and non-AMP pairs will be collected using their cross-link as done in our AMP work [7], securing as diverse publishers as possible. As an AMP and non-AMP pair basically convey the same contents but their optimization degree is different, each version can be used as a control and testing case of different PFP policies to compare the gap.

For the performance metrics, the core metrics in Web Vitals [18], which is, Largest Contentful Paint (LCP), First Input Delay(FID), Cumulative Layout Shift (CLS), will be used instead of traditional metrics used in AMP work [7] such as Page Load Time (PLT) and Time to First Bytes. Web Vitals is a recently suggested initiative to portray web performance more effectively. Specifically, LCP represents loading per-formance better than PLT, as the swift presentation of meaningful content is remarkably crucial [19] but PLT cannot show it. Besides, CLS, which shows how the page is visually stable, is also important to measure, as the more frequent layout shift will end up in a delay of page loading.

4.2	Measurement design

In this study, it is crucial to test as diverse user conditions (i.e., different devices and network configuration) as possible to classify and/or cluster them. The best option to have such various conditions is to collaborate with


1	There are more than 24 thousands mobile devices only for Android, as of 2015 [17]
 


4
 















Figure 3: Measurement tool design


a Content Delivery Network (CDN). CDN is a party in favor of providing better performance, as it is what their customers prefer, and our research will give them an opportunity to provide customized performance optimization to its customer. Our system implemented in CDN will modify a PFP header and perform an AB test per page, collecting user’s conditions as well as test results utilizing the report from Real User Monitoring (RUM) tool such as Google Analytics or Akamai’s mPulse. Alternatively, crowdsourced testing can be conducted with a Chrome extension that can manipulate Permissions Policy. As the size of the user pool of a Chrome extension is significantly smaller than CDN’s, the users of the crowdsourced test will be cautiously separated into two classes; passive users and active users. The passive users will be monitored like the test in CDN for further classification. The clear incentive for passive users is the capability to leverage PFP features on their browser for better performance. On the other hand, the active users will perform AB testings in their device for multiple pages and performance features and be paid for their participation in the research. A set of AMP and non-AMP pairs with different Permissions Policy will be loaded on their browser, and the test results, along with their device spec and general network status, will be reported 2. The combination of distinct webpages, user devices, network configuration, and a Permissions Policy set for the best performance will be the results of our test. As the complete combination of such conditions is limitless, we will focus on a few policy sets as discussed in Sec. 3.1 and a finite set of webpages (Sec. 4.1).

4.3	Tool design

PFP will perfectly work when implemented in the browser core. With the lack of such authority, however, we will build a dedicated tool, either one for CDN or a Chrome extension. As tool design for CDN depends on their structure and the degree of cooperation, and the basic functionality of the tool would be the same, we describe the Chrome extension design here. We carefully selected Chrome extension as Chrome follows the evolution of Permissions Policy [14]. We are building a Chrome extension that instrument PFP features by either modifying the HTTP header for the entire page or allow attribute for the iframe for the measurement (Fig. 3) 3. Whenever a web page requested delivered from the server, the extension injects a set of PFP tags in the HTTP header. Some tests, which require the limited control on the target content such as a test for third-party contents, will use iframe attribute modifier instead of HTTP header modification. The extension will monitor the performance and report to the server with the Performance observer. For the active users


2	This test will be done when the app is in the foreground to minimize the performance degradation caused by the other apps. Also, the testing will not be executed when the browser is actively loading the other page by the user request.
3 A limitation on mobile Chrome is that it does not supports the extensions for the desktop Chrome. Fortunately, we can use a mobile browser that support Chrome extensions, Kiwi Browser, which is based on the latest Chrome.
 


5
 
discussed in the previous subsection, a dedicated tester function will run on the user’s device to test target AMP and non-AMP pairs with differently throttled with the performance tags in PFP.

